Seismic Signatures of the $^{12}$C($\alpha$, $\gamma$)$^{16}$O Reaction Rate in White Dwarf Models with Overshooting

We consider the combined effects that overshooting and the $^{12}$C($\alpha$, $\gamma$)$^{16}$O reaction rate have on variable white dwarf stellar models. We find that carbon-oxygen white dwarf models continue to yield pulsation signatures of the current experimental $^{12}$C($\alpha$, $\gamma$)$^{16}$O reaction rate probability distribution function when overshooting is included in the evolution. These signatures hold because the resonating mantle region, encompassing $\simeq$\,0.2\,\Msun\ in a typical $\simeq$\,0.6\,\Msun\ white dwarf model, still undergoes radiative helium burning during the evolution to a white dwarf. Our specific models show two potential low-order adiabatic g-modes, $g_2$ and $g_6$, that signalize the $^{12}$C($\alpha$, $\gamma$)$^{16}$O reaction rate probability distribution function. Both g-mode signatures induce average relative period shifts of $\Delta P/P = 0.44 \%$ and $\Delta P/P = 1.33\%$ for $g_2$ and $g_6$ respectively. We find that $g_6$ is a trapped mode, and the $g_2$ period signature is inversely proportional to the $^{12}$C($\alpha$, $\gamma$)$^{16}$O reaction rate. The $g_6$ period signature generally separates the slower and faster reaction rates, and has a maximum relative period shift of $\Delta P/P = 3.45\%$. We conclude that low-order g-mode periods from carbon-oxygen white dwarfs may still serve as viable probes for the $^{12}$C($\alpha$, $\gamma$)$^{16}$O reaction rate probability distribution function when overshooting is included in the evolution.

==> macros/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\bvec{\nabla} \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex
